Stellar- and AGN-Driven Outflows in JWST Galaxies at z=3-9: More Frequent, Wider Opening Angles, and Mostly Bounded

We study outflows in 130 galaxies with -22<MUV<-16 at z=3-9 identified in JWST NIRSpec and NIRCam WFSS data taken by the ERO, CEERS, FRESCO, GLASS, and JADES programs. We identify 30 out of the 130 galaxies with broad components of FWHM~200-700 km s$^{-1}$ in the emission lines of H${\alpha}$ and [OIII] that trace ionized outflows, and find no excesses from the star-formation main sequence. Four out of the 30 outflowing galaxies are Type-1 AGN whose H${\alpha}$ emission lines include line profile components as broad as FWHM>1000 km s$^{-1}$ while one galaxy is identified as a Type-2 AGN by high ionization emission lines. With the velocity shift and line widths of the outflow broad lines, we obtain ~80-500 km s$^{-1}$ for the outflow velocities. We find that the outflow velocities are slower than low-z galaxies with similar SFRs, which may be explained by the low stellar masses of high-z galaxies. The outflow velocities of AGNs are large but not significantly different from the others. Interestingly, these outflow velocities are typically not high enough to escape from the galactic potentials, possibly suggesting fountain-type outflows. We estimate mass loading factors ${\eta}$ to be 0.1-1 that are not particularly large, but comparable with those of z~1 outflows. The large fraction of galaxies with outflows (30% with high resolution data) provides constraints on outflow parameters, suggesting a wide opening angle of >45 deg and a large duty-cycle of >30%, which gives a picture of more frequent and spherical outflows in high-z galaxies.

==> FRESCO_objects_tab.tex <==
FRESCO N \#1 & 12:36:37.90 & 62:18:08.78 & 7.505 & $156.52\pm11.56$ \\
FRESCO N \#2 & 12:36:37.86 & 62:18:08.60 & 7.501 & $162.11\pm10.94$ \\
FRESCO N \#3 & 12:37:04.80 & 62:17:18.82 & 7.637 & $280.39\pm17.86$ \\
FRESCO N \#4 & 12:36:54.03 & 62:17:10.67 & 7.974 & $61.85\pm7.40$ \\
FRESCO N \#5 & 12:36:48.88 & 62:16:06.50 & 7.094 & $71.89\pm9.91$ \\
FRESCO N \#6 & 12:36:59.91 & 62:14:28.41 & 7.144 & $122.34\pm10.87$ \\
FRESCO N \#7 & 12:37:19.94 & 62:15:26.04 & 7.591 & $287.28\pm19.54$ \\
FRESCO S \#1 & 03:32:21.00 & -27:48:53.55 & 7.848 & $104.90\pm10.74$ \\
FRESCO S \#2 & 03:32:27.25 & -27:47:36.54 & 7.166 & $84.73\pm9.85$ \\
FRESCO S \#3\footnote{possible $z=1.7$ interloper} & 03:32:32.91 & -27:45:37.45 & 8.019 & $133.22\pm10.10$ \\
FRESCO S \#4 & 03:32:46.90 & -27:50:07.60 & 7.275 & $248.55\pm17.12$ \\
FRESCO S \#5 & 03:32:41.42 & -27:44:38.18 & 7.573 & $125.26\pm11.10$
